An Empirical Study of Challenges in Converting Deep Learning Models

There is an increase in deploying Deep Learning (DL)-based software systems in real-world applications. Usually DL models are developed and trained using DL frameworks that have their own internal mechanisms/formats to represent and train DL models, and usually those formats cannot be recognized by other frameworks. Moreover, trained models are usually deployed in environments different from where they were developed. To solve the interoperability issue and make DL models compatible with different frameworks/environments, some exchange formats are introduced for DL models, like ONNX and CoreML. However, ONNX and CoreML were never empirically evaluated by the community to reveal their prediction accuracy, performance, and robustness after conversion. Poor accuracy or non-robust behavior of converted models may lead to poor quality of deployed DL-based software systems. We conduct, in this paper, the first empirical study to assess ONNX and CoreML for converting trained DL models. In our systematic approach, two popular DL frameworks, Keras and PyTorch, are used to train five widely used DL models on three popular datasets. The trained models are then converted to ONNX and CoreML and transferred to two runtime environments designated for such formats, to be evaluated. We investigate the prediction accuracy before and after conversion. Our results unveil that the prediction accuracy of converted models are at the same level of originals. The performance (time cost and memory consumption) of converted models are studied as well. The size of models are reduced after conversion, which can result in optimized DL-based software deployment. Converted models are generally assessed as robust at the same level of originals. However, obtained results show that CoreML models are more vulnerable to adversarial attacks compared to ONNX.

==> Qiang.tex <==
\subsection{RQ??: Qiang's work}
\Amin{please write down your experiments here, thank you}
In this experiment, we selected the CIFAR-10 dataset and trained three CNN models using PyTorch, namely VGG, ResNet, and AlexNet. We then converted those models to ONNX and evaluated the inference time and the average absolute difference in raw output of the converted model with respect to the original model.
After converting each PyTorch model to ONNX, we imported it into ONNX runtime, Caffe2 and TensorFlow backends for inference. The overall test set accuracy is the same and the raw output values have differences in decimal places. The inference time varies according to backend used while the raw output values have tendency to vary according to model architecture.
Figure \ref{fig:q} and \ref{fig:Q_raw_output_error}.

\begin{figure}[t]
%\scalebox{0.70}{
\center
\includegraphics[width=\linewidth]{images/inference_time.pdf}
\caption{inference time}
\label{fig:Q_inference_time}
%}
\end{figure}

\begin{figure}[t]
%\scalebox{0.70}{
\center
\includegraphics[width=\linewidth]{images/raw_output_error.pdf}
\caption{raw output error}
\label{fig:Q_raw_output_error}
%}
\end{figure}

==> pdf/errors/subplots-coreml.tex <==

\begin{figure*}
%\begin{adjustbox}{width=0.75\columnwidth,center}
    \scalebox{1}{   
        \begin{subfigure}[b]{0.4\textwidth}
            \includegraphics[width=\linewidth]{pdf/errors/coreml/lenet5-absolute-errors-coreml.pdf}
            \caption{Lenet5 absolute errors)}
            \label{fig:sub-assembly1}
        \end{subfigure}%
        \begin{subfigure}[b]{0.4\textwidth}
            \includegraphics[width=\linewidth]{pdf/errors/coreml/lenet5-relative-errors-coreml.pdf}
            \caption{lenet5-relative-errors}
            \label{fig:sub-assembly2}
        \end{subfigure}%
        \hfill
    %\caption{Pictures of animals}\label{fig:animals}
    }
	
	
	\scalebox{1}{ 
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\linewidth]{pdf/errors/coreml/resnet18-absolute-errors-coreml.pdf}
        \caption{resnet18-absolute-error}
        \label{fig:sub-Annealing1}
    \end{subfigure}%
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\linewidth]{pdf/errors/coreml/resnet18-relative-errors-coreml.pdf}
        \caption{resnet18-relative-errors}
        \label{fig:sub-Annealing2}
    \end{subfigure}
    \hfill
    }
        %%% row2
       % 
       % \scalebox{1}{ 
       %  \begin{subfigure}[b]{0.4\textwidth}
                %\includegraphics[width=\linewidth]{pdf/errors/coreml/vgg-absolute-errors-coreml.pdf}
                %\caption{vgg-absolute-errors}
                %\label{fig:sub-Experimentation1}
       % \end{subfigure}%
       % \begin{subfigure}[b]{0.4\textwidth}
                %\includegraphics[width=\linewidth]{pdf/errors/coreml/vgg-absolute-errors-coreml.pdf}
                %\caption{vgg-absolute-errors}
                %\label{fig:sub-Experimentation2}
       % \end{subfigure}%
       % }
        %\hfill
        \scalebox{1}{ 
        \begin{subfigure}[b]{0.4\textwidth}
                \includegraphics[width=\linewidth]{pdf/errors/coreml/lstm-absolute-errors-coreml.pdf}
                \caption{lstm-absolute-errors}
                \label{fig:sub-Full-stack1}
        \end{subfigure}%
        \begin{subfigure}[b]{0.4\textwidth}
                \includegraphics[width=\linewidth]{pdf/errors/coreml/lstm-relative-errors-coreml.pdf}
                \caption{lstm-relative-errors}
                \label{fig:sub-Full-stack2}
        \end{subfigure}
          }
        %%%%%% row 3
        
        %\hfill
        \scalebox{1}{ 
         \begin{subfigure}[b]{0.4\textwidth}
                \includegraphics[width=\linewidth]{pdf/errors/coreml/gru-absolute-errors-coreml.pdf}
                \caption{gru-absolute-errors}
                \label{fig:sub-Chemistry1}
        \end{subfigure}%
        \begin{subfigure}[b]{0.4\textwidth}
                \includegraphics[width=\linewidth]{pdf/errors/coreml/gru-relative-errors-coreml.pdf}
                \caption{gru-relative-errors}
                \label{fig:sub-Chemistry2}
        \end{subfigure}%
        }
        
        \caption{The Absolute and Relative errors of the DL models when converted from the respective framework to coreml runtime.}
        
    \label{fig:error-onnx-coreml} 
\end{figure*}

==> pdf/errors/subplots-onnx.tex <==

\begin{figure*}
%\begin{adjustbox}{width=0.75\columnwidth,center}
    \scalebox{1}{   
        \begin{subfigure}[b]{0.4\textwidth}
            \includegraphics[width=\linewidth]{pdf/errors/onnx/lenet5-absolute-errors-onnx.pdf}
            \caption{Lenet5 absolute errors%\Amin{after conversion? are they average of 10 models?}
            }
            \label{fig:sub-assembly1}
        \end{subfigure}%
        \begin{subfigure}[b]{0.4\textwidth}
            \includegraphics[width=\linewidth]{pdf/errors/onnx/lenet5-relative-errors-onnx.pdf}
            \caption{lenet5-relative-errors}
            \label{fig:sub-assembly2}
        \end{subfigure}%
        \hfill
    %\caption{Pictures of animals}\label{fig:animals}
    }
	
	
	\scalebox{1}{ 
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\linewidth]{pdf/errors/onnx/resnet18-absolute-errors-onnx.pdf}
        \caption{resnet18-absolute-errors}
        \label{fig:sub-Annealing1}
    \end{subfigure}%
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\linewidth]{pdf/errors/onnx/resnet18-relative-errors-onnx.pdf}
        \caption{resnet18-relative-errors}
        \label{fig:sub-Annealing2}
    \end{subfigure}
    \hfill
    }
        %%% row2
       % 
       % \scalebox{1}{ 
       %  \begin{subfigure}[b]{0.4\textwidth}
                %\includegraphics[width=\linewidth]{pdf/errors/onnx/vgg-absolute-errors-onnx.pdf}
                %\caption{vgg-absolute-errors}
                %\label{fig:sub-Experimentation1}
       % \end{subfigure}%
       % \begin{subfigure}[b]{0.4\textwidth}
                %\includegraphics[width=\linewidth]{pdf/errors/onnx/vgg-absolute-errors-onnx.pdf}
                %\caption{vgg-absolute-errors}
                %\label{fig:sub-Experimentation2}
       % \end{subfigure}%
       % }
        %\hfill
        \scalebox{1}{ 
        \begin{subfigure}[b]{0.4\textwidth}
                \includegraphics[width=\linewidth]{pdf/errors/onnx/lstm-absolute-errors-onnx.pdf}
                \caption{lstm-absolute-errors}
                \label{fig:sub-Full-stack1}
        \end{subfigure}%
        \begin{subfigure}[b]{0.4\textwidth}
                \includegraphics[width=\linewidth]{pdf/errors/onnx/lstm-relative-errors-onnx.pdf}
                \caption{lstm-relative-errors}
                \label{fig:sub-Full-stack2}
        \end{subfigure}
          }
        %%%%%% row 3
        
        %\hfill
        \scalebox{1}{ 
         \begin{subfigure}[b]{0.4\textwidth}
                \includegraphics[width=\linewidth]{pdf/errors/onnx/gru-absolute-errors-onnx.pdf}
                \caption{gru-absolute-errors}
                \label{fig:sub-Chemistry1}
        \end{subfigure}%
        \begin{subfigure}[b]{0.4\textwidth}
                \includegraphics[width=\linewidth]{pdf/errors/onnx/gru-relative-errors-onnx.pdf}
                \caption{gru-relative-errors}
                \label{fig:sub-Chemistry2}
        \end{subfigure}%
        }
        
        \caption{The Absolute and Relative errors of the DL models when converted from the respective framework to onnx runtime.}
        
    \label{fig:error-onnx-runtime}       
\end{figure*}


==> pdf/runtime/memory/plot-memory.tex <==
\begin{figure*}
\centering
        \begin{subfigure}[b]{0.5\textwidth}
            \includegraphics[width=\linewidth]{pdf/runtime/memory/lenet5-memory-batch-128.pdf}
            \caption{Lenet5}
            \label{fig:sub-assembly1}
        \end{subfigure}%
   \hfill
    \begin{subfigure}[b]{0.5\textwidth}
        \includegraphics[width=\linewidth]{pdf/runtime/memory/resnet18-memory-batch-128.pdf}
        \caption{Resnet18}
        \label{fig:sub-Annealing1}
    \end{subfigure}%

    \hfill
 
    \begin{subfigure}[b]{0.5\textwidth}
                \includegraphics[width=\linewidth]{pdf/runtime/memory/lstm-memory-batch-128.pdf}
                \caption{lstm}
                \label{fig:sub-Full-stack1}
    \end{subfigure}%
    \hfill
     \begin{subfigure}[b]{0.5\textwidth}
                \includegraphics[width=\linewidth]{pdf/runtime/memory/gru-memory-batch-128.pdf}
                \caption{GRU}
                \label{fig:sub-Full-stack1}
    \end{subfigure}%
        
    \caption{Memory usage for DL models in different frameworks and runtime environments.}
    \label{fig:memory}
       
\end{figure*}

==> pdf/runtime/time/plot_inference-time.tex <==
\begin{figure*}
    \begin{subfigure}[b]{0.5\textwidth}
            \includegraphics[width=\linewidth]{pdf/runtime/time/lenet5-inference-batch-128.pdf}
            \caption{Lenet5}
            \label{fig:sub-assembly1}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[b]{0.5\textwidth}
        \includegraphics[width=\linewidth]{pdf/runtime/time/resnet18-inference-batch-128.pdf}
        \caption{Resnet18}
        \label{fig:sub-Annealing1}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[b]{0.5\textwidth}
                \includegraphics[width=\linewidth]{pdf/runtime/time/lstm-inference-batch-128.pdf}
                \caption{lstm}
                \label{fig:sub-Full-stack1}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[b]{0.5\textwidth}
                \includegraphics[width=\linewidth]{pdf/runtime/time/gru-inference-batch-128.pdf}
                \caption{GRU}
                \label{fig:sub-Full-stack1}
    \end{subfigure}%
    
    \caption{The inference time of DL models in different frameworks and runtime environments.}
    \label{fig:inference-time}
\end{figure*}

==> pdf/training/plot-training-validation.tex <==

\begin{figure}
%\begin{adjustbox}{width=0.75\columnwidth,center}
    %\scalebox{1}{   
        \begin{subfigure}[b]{0.5\textwidth}
            \includegraphics[width=\linewidth]{pdf/training/Resnet5-Training.pdf}
            \caption{Resnet18 training)}
            \label{fig:sub-assembly1}
        \end{subfigure}%
   
        \hfill
    %\caption{Pictures of animals}\label{fig:animals}
   % }
	
	
	%\scalebox{1}{ 
    \begin{subfigure}[b]{0.5\textwidth}
        \includegraphics[width=\linewidth]{pdf/training/Lenet5-Training.pdf}
        \caption{Lenet5 Training}
        \label{fig:sub-Annealing1}
    \end{subfigure}%

    \hfill
    %}
        %%% row2
       % 
       % \scalebox{1}{ 
       %  \begin{subfigure}[b]{0.4\textwidth}
                %\includegraphics[width=\linewidth]{pdf/errors/onnx/vgg-absolute-errors-onnx.pdf}
                %\caption{vgg-absolute-errors}
                %\label{fig:sub-Experimentation1}
       % \end{subfigure}%
       % \begin{subfigure}[b]{0.4\textwidth}
                %\includegraphics[width=\linewidth]{pdf/errors/onnx/vgg-absolute-errors-onnx.pdf}
                %\caption{vgg-absolute-errors}
                %\label{fig:sub-Experimentation2}
       % \end{subfigure}%
       % }
        %\hfill
        %\scalebox{1}{ 
        \begin{subfigure}[b]{0.5\textwidth}
                \includegraphics[width=\linewidth]{pdf/training/Lstm-Training.pdf}
                \caption{Lstm-Training}
                \label{fig:sub-Full-stack1}
        \end{subfigure}%
        
        \caption{The Training accuracy of the DL models across ten training circles.}
       
    \end{figure}
    
    
    
    
    
    
    \begin{figure}
%\begin{adjustbox}{width=0.75\columnwidth,center}
    %\scalebox{1}{   
      
        \begin{subfigure}[b]{0.5\textwidth}
            \includegraphics[width=\linewidth]{pdf/training/Resnet18-Validation.pdf}
            \caption{Resnet18 validation}
            \label{fig:sub-assembly2}
        \end{subfigure}%
        \hfill
    %\caption{Pictures of animals}\label{fig:animals}
   % }
	
	
	%\scalebox{1}{ 
  
    \begin{subfigure}[b]{0.5\textwidth}
        \includegraphics[width=\linewidth]{pdf/training/Lenet5-Validation.pdf}
        \caption{Lenet5-Validation}
        \label{fig:sub-Annealing2}
    \end{subfigure}
    \hfill
    %}
        %%% row2
       % 
       % \scalebox{1}{ 
       %  \begin{subfigure}[b]{0.4\textwidth}
                %\includegraphics[width=\linewidth]{pdf/errors/onnx/vgg-absolute-errors-onnx.pdf}
                %\caption{vgg-absolute-errors}
                %\label{fig:sub-Experimentation1}
       % \end{subfigure}%
       % \begin{subfigure}[b]{0.4\textwidth}
                %\includegraphics[width=\linewidth]{pdf/errors/onnx/vgg-absolute-errors-onnx.pdf}
                %\caption{vgg-absolute-errors}
                %\label{fig:sub-Experimentation2}
       % \end{subfigure}%
       % }
        %\hfill
        %\scalebox{1}{ 
       
        \begin{subfigure}[b]{0.5\textwidth}
                \includegraphics[width=\linewidth]{pdf/training/Lstm-Validation.pdf}
                \caption{Lstm-Validation}
                \label{fig:sub-Full-stack2}
        \end{subfigure}
        
        \caption{The Validation accuracy of the DL models across ten \Amin{or nine?} training circles.}
       
    \end{figure}


==> tables/RQ1/tbl_conversion_errors.tex <==
%\newline
\begin{table}[t]
\caption{Comparison of the conversion error rate \Amin{do you mean the error in prediction accuracy after conversion?} of different DL models across the selected DL frameworks}

 %   \tiny
 %   
    
%    \label{subtab:resnet18}

    \begin{adjustbox}{width=0.5\textwidth,center}
    \begin{tabular}{c| m{1.6cm} m{1.6cm}| m{1.6cm} m{1.6cm}| m{1.6cm} m{1.6cm}| m{1.6cm} m{1.6cm}  }\toprule
    
    %\caption{The conversion errors, prediction time and model for DNN model before and when converted from the respective ML frameworks to onnx format; given the similar input test data of 10,000 sample size. } 
    
    %\rowcolor{gray!15}
    &\multicolumn{2}{c|}{\textbf{Keras}}&\multicolumn{2}{c|}{\textbf{Pytorch}} & \multicolumn{2}{c|}{\textbf{MXNET}}  & \multicolumn{2}{c}{\textbf{CNTK}}\\ %\hline
    
    \rowcolor{gray!15}
    &\multicolumn{2}{c|}{\textbf{Avg. Error (std)}}&\multicolumn{2}{c|}{\textbf{Avg. Error (std)}} & \multicolumn{2}{c|}{\textbf{Avg. Error (std)}}  & \multicolumn{2}{c}{\textbf{Avg. Error (std)}}\\ %\midrule
    
    \rowcolor{gray!15}
   \textbf{Model}&\textbf{Abs}&\textbf{Rel}
    &\textbf{Abs}&\textbf{Rel}&\textbf{Abs}&\textbf{Rel}&\textbf{Abs}&\textbf{Rel}\\ \midrule
    
    %Alexnet
     Alexnet& & & & & & & \\ %hline
       \rowcolor{gray!10}
     Lenet5&7.45e-08 (2.079e-08) &9.76e-07 (2.725e-07) & 9.54e-07 (1.185e-06) &1.16E-07 (5.893e-07) &&& & \\ %hline
      %\rowcolor{gray!10}
     Resnet18&5.07e-07 (2.461e-07) &1.11e-06 (5.530e-07)&2.38e-06 (2.772e-06) &7.61e-07 (8.205e-07)&&& &\\ %hline
      \rowcolor{gray!10}
     Resnet50& &&1.96e-05 (2.434e-05) &4.63e-06 (1.006e-05)&&& &\\ %hline
     
     VGG&3.73e-08 (3.145e-08) &1.63e-07 (1.331e-07)& &&&&& \\ %hline
     
      \rowcolor{gray!10}
     LSTM&1.79e-08 (9.670e-08)&7.76e-07 (1.018e-1)& 3.422e-08 (5.027e-08)&1.196e-07 (1.853e-06)&&&& \\ 
     
     GRU&7.230e-12 (3.482e-07) &0 (8.466e-02)&3.864e-08 (4.043e-08) &1.413e-07 (8.716e-07)&&&& \\ %\hline
    \bottomrule
    %\vspace{-5pt}
    \end{tabular}  
    %}
    \end{adjustbox}
    %}
\end{table}



%% Issues
% InvalidGraph: [ONNXRuntimeError] : 10 : INVALID_GRAPH : Load model from ./data/ONNX/keras/keras-tf_resnet50-mnist.onnx failed:This is an invalid model. Type Error: Type 'tensor(uint8)' of input parameter (Resize__634:0) of operator (Conv) in node (Conv__1061) is invalid.



%%% training LSTM in keras
% NotImplementedError: Cannot convert a symbolic Tensor (lstm_1/strided_slice:0) to a numpy array. This error may indicate that you're trying to pass a Tensor to a NumPy call, which is not supported






%%%% Errors while exporting back the modl from onnx to pytorch

%1- NotImplementedError: OpCodeGenerator is unimplemented for GRU.
%2 - NotImplementedError: OpCodeGenerator is unimplemented for LSTM.

%% converting VGG: TypeError: __init__() missing 2 required positional arguments: 'in_channels' and 'out_channels'

%% Conversion in mxnet to onnx
% ImportError: Onnx and protobuf need to be installed. Instructions to install - https://github.com/onnx/onnx

%% ONNX doesn't have "pooling_convention" attribute for pooling(Max/Avg) #549


%% Converting VGG in torch: RuntimeError: Unsupported: ONNX export of operator adaptive_avg_pool2d, since output size is not factor of input size. Please feel free to request support or submit a pull request on PyTorch GitHub.

==> tables/sub/sub_resnet18.tex <==
%\newline
\begin{table*}[t]
\caption{Comparison of ... \Amin{can we have standard deviations as well?}\Amin{Moreover, are these results after conversion, or before?}\\ \Moses{Sure I can add the standard deviations. The errors are is the difference between before and after the conversion. the Time is the avg total time took during the conversion. Time1 is the prediction time before  and Time2 is the prediction time after conversion to onnx. similarly, the size1 is the model size before and size2 is after converting to onnx }}

 %   \tiny
 %   
    
%    \label{subtab:resnet18}

    \begin{adjustbox}{width=0.75\textwidth,center}
    \begin{tabular}{c| c| r r| r r r | r r  }\toprule
    
    %\caption{The conversion errors, prediction time and model for DNN model before and when converted from the respective ML frameworks to onnx format; given the similar input test data of 10,000 sample size. } 
    
    \rowcolor{gray!15}
    &&\multicolumn{2}{c|}{\textbf{Avg. Error}}&\multicolumn{3}{c|}{\textbf{Avg. Time}} & \multicolumn{2}{c}{\textbf{Model size}}\\ %\midrule
    \rowcolor{gray!15}
   \textbf{Model}&\textbf{Framework}&\textbf{Abs}&\textbf{Rel}
    &\textbf{Time}&\textbf{Time1}&\textbf{Time2}&\textbf{Size1}&\textbf{Size2}\\ \midrule
    
    %Alexnet
     \multirow{6}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1cm}{\centering \textbf{Alexnet}}}} 
    & Keras& && &&&11,730,736&\\ %hline
    & Pytorch& 3.706e-04&2.774e-03& 4.5906 &0.0124&2.6253&&\\ %hline
    & MXNet& && &&&\\ %hline
    & CNTK& && &&&\\ %hline
    & CoreML& && &&&\\ %hline
    & Sklearn& && &&&\\ \hline
    
    %Lenet-5
     \multirow{6}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1cm}{\centering \textbf{Lenet5}}}} 
    & Keras&7.219e-07 &1.960e-03& 0.3793&0.0888&0.0334&601,872&\\ %hline
    & Pytorch&1.34E-05 &9.78E-04 &0.0943& 0.0035&0.0398&&\\ %hline
    & MXNet& && &&&\\ %hline
    & CNTK& && &&&\\ %hline
    & CoreML& && &&&\\ %hline
    & Sklearn& && &&&\\ \hline
    
    %Resnet18
     \multirow{6}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1cm}{\centering \textbf{Resnet18}}}} 
    & Keras&1.167e-06 &4.487e-06 &11.5937& 0.6044&3.7775&89,756,056&44,688,722\\ %hline
    & Pytorch&1.720e-05 &9.370e-03&1.6389 &0.0808&0.6923&&\\ %hline
    & MXNet& && &&&\\ %hline
    & CNTK& && &&&\\ %hline
    & CoreML& && &&&\\ %hline
    & Sklearn& && &&&\\ \hline
    
    
    %Resnet50
     \multirow{6}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1cm}{\centering \textbf{Resnet50}}}} 
    & Keras& && &&&159,300,984&\\ %hline
    & Pytorch& 2.607e-04&2.575e-02& 5.7136&0.1833&1.9535&&\\ %hline
    & MXNet& && &&&\\ %hline
    & CNTK& && &&&\\ %hline
    & CoreML& && &&&\\ %hline
    & Sklearn& && &&&\\ \hline
    
    
    %VGG
     \multirow{6}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1cm}{\centering \textbf{VGG}}}} 
    & Keras&3.017e-07 &1.383e-06&8.9313 &0.5867&1.9758&71,945,464&35,824,142\\ %hline
    & Pytorch& && &&&\\ %hline
    & MXNet& && &&&\\ %hline
    & CNTK& && &&&\\ %hline
    & CoreML& && &&&\\ %hline
    & Sklearn& && &&&\\ \hline
    
    %LSTM
     \multirow{6}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1cm}{\centering \textbf{LSTM}}}} 
    & Keras& && &&&144,762,352&48,256,816\\ %hline
    & Pytorch&1.808e-07 &6.0367e-06&0.1252 &0.0215&0.5175&\\ %hline
    & MXNet& && &&&\\ %hline
    & CNTK& && &&&\\ %hline
    & CoreML& && &&&\\ %hline
    & Sklearn& && &&&\\ 
    
    \bottomrule
    %\vspace{-5pt}
    \end{tabular}  
    %}
    \end{adjustbox}
    %}
\end{table*}



%% Issues
% InvalidGraph: [ONNXRuntimeError] : 10 : INVALID_GRAPH : Load model from ./data/ONNX/keras/keras-tf_resnet50-mnist.onnx failed:This is an invalid model. Type Error: Type 'tensor(uint8)' of input parameter (Resize__634:0) of operator (Conv) in node (Conv__1061) is invalid.



%%% training LSTM in keras
% NotImplementedError: Cannot convert a symbolic Tensor (lstm_1/strided_slice:0) to a numpy array. This error may indicate that you're trying to pass a Tensor to a NumPy call, which is not supported






%%%% Errors while exporting back the modl from onnx to pytorch

%1- NotImplementedError: OpCodeGenerator is unimplemented for GRU.
%2 - NotImplementedError: OpCodeGenerator is unimplemented for LSTM.

%% converting VGG: TypeError: __init__() missing 2 required positional arguments: 'in_channels' and 'out_channels'

%% Conversion in mxnet to onnx
% ImportError: Onnx and protobuf need to be installed. Instructions to install - https://github.com/onnx/onnx

%% ONNX doesn't have "pooling_convention" attribute for pooling(Max/Avg) #549

==> tables/table1.tex <==
\begin{table*}
\caption{Benchmark hyparameter and number of iteration}
\label{validationTable}
%\resizebox{.99\textwidth}{!}{
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|}
\hline

\multirow{2}{*}{\textbf{Model}} & Batch size & Training epochs &conversion epochs & & & High impact \\
& 1 & 2 & 3 & 4 & 5 \\

\hline %% sorrry let me create a copy! ok!
Does the bug impact a UI element? & X & & & & \\

\hline
Does the bug impact information about the model? & X & X & X & & \\

\hline
Does the bug alter part of the network operation? & & & X & X & X \\

\hline
Does the bug change the result of the network?  & & & & X & X\\
\hline
\end{tabular}
\end{center}
\label{table:table-1}
%}
\end{table*}

==> tables/tbl_accuracy_old.tex <==
\begin{table}[t!]
    \large
    \caption{The average prediction accuracy and the average inference time over the testing datasets for DL model after training per framework\Amin{to be updated!}.}
    
    \label{tab:projects_category}

    \begin{adjustbox}{width=0.9\linewidth,center}
         \begin{tabular}{c| c c| c c}%\toprule
    
    \multirow{2}{*}{\textbf{Model}} &\multicolumn{2}{c|}{\textbf{Keras}}& \multicolumn{2}{c}{\textbf{PyTorch}}\\ %\midrule
    %\rowcolor{gray!15}
    %% Keras
    &\textbf{Accuracy}& 
    %% Pytorch
     \textbf{Time (sec.)}& 
    %% MXNet
     \textbf{Accuracy}& 
    %% CNTK
     \textbf{Time (sec.)} 
    %% Sklearn
    \\ %\midrule
    \rowcolor{gray!15}
    %% Keras
    %\midrule
    \hline
    %\rowcolor{gray!10}
    LeNet-5& 99.4 & 0.0533 & 99.1 & 0.0257\\ %hline
    %\rowcolor{gray!10}
    ResNet-18& 67.8&1.4439 &83.8 & 0.5217\\ %hline
    
    \rowcolor{gray!10}
    VGG-16& 77.5& 0.7610& 76.6& 0.8552\\ %hline
    %\rowcolor{gray!10}
    LSTM& 88.3& 0.1775& 84.8& 3.7945\\ %hline
    
    \rowcolor{gray!10}
    GRU&88.8 & 0.1669& 86.0& 3.5499\\ %hline
    %\bottomrule
    %\vspace{-5pt}
    \end{tabular}  
    %}
    \end{adjustbox}
    %}
\end{table}

==> tables/tbl_conversion.tex <==
\begin{table}
\caption{Effort required to fix technical debts in terms of debt types and severity types.}
%\caption{Distribution of the required effort (the time in minutes) to fix issues in a category. 
%\mehdi{I think we can move the description highlighted with red to the text, not in the caption of table.} \textcolor{red}{We analyzed the effort both on the issue types (\emph{SQ-Bug} or \emph{Code Smell}) and their severity(\emph{critical, major, blocker, or minor}).  We report the mean percentage values across the projects in a category.  $\sigma$ denotes the standard deviation of the percentage values across the projects in a category.} } 
\label{tab:issue-types}

	\centering
	%\scalebox{0.65}{
	\begin{adjustbox}{width=0.40\textwidth,center}
	\begin{subtable}[t]{0.5\textwidth}
		%\caption{Effort required to fix technical debts in terms of the debt types (coding errors and code smells)}	
		\label{subtab:effort_type}
		\centering
        
    \begin{tabular}{c| c| r r| r r | r r  }\toprule
    
    %\caption{The conversion errors, prediction time and model for DNN model before and when converted from the respective ML frameworks to onnx format; given the similar input test data of 10,000 sample size. } 
    
    \rowcolor{gray!15}
    &&\multicolumn{2}{c|}{\textbf{Error Rate}}&\multicolumn{2}{c|}{\textbf{Time}} & \multicolumn{2}{c}{\textbf{Model size}}\\ %\midrule
    \rowcolor{gray!15}
   \textbf{Model}&\textbf{Framework}&\textbf{Abs}&\textbf{Rel}
    &\textbf{Time1}&\textbf{Time2}&\textbf{Size1}&\textbf{Size2}\\ \midrule
    
    %Alexnet
     \multirow{6}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1cm}{\centering \textbf{Alexnet}}}} 
    & Keras& && &&\\ %hline
    & Pytorch& && &&\\ %hline
    & MXNet& && &&\\ %hline
    & CNTK& && &&\\ %hline
    & CoreML& && &&\\ %hline
    & Sklearn& && &&\\ \hline
    
    %Lenet-5
     \multirow{6}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1cm}{\centering \textbf{Lenet5}}}} 
    & Keras& && &&\\ %hline
    & Pytorch& && &&\\ %hline
    & MXNet& && &&\\ %hline
    & CNTK& && &&\\ %hline
    & CoreML& && &&\\ %hline
    & Sklearn& && &&\\ \hline
    
    %Resnet18
     \multirow{6}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1cm}{\centering \textbf{Resnet18}}}} 
    & Keras& && &&\\ %hline
    & Pytorch& && &&\\ %hline
    & MXNet& && &&\\ %hline
    & CNTK& && &&\\ %hline
    & CoreML& && &&\\ %hline
    & Sklearn& && &&\\ \hline
    
    
    %Resnet50
     \multirow{6}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1cm}{\centering \textbf{Resnet50}}}} 
    & Keras& && &&\\ %hline
    & Pytorch& && &&\\ %hline
    & MXNet& && &&\\ %hline
    & CNTK& && &&\\ %hline
    & CoreML& && &&\\ %hline
    & Sklearn& && &&\\ \hline
    
    
    %VGG
     \multirow{6}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1cm}{\centering \textbf{VGG}}}} 
    & Keras& && &&\\ %hline
    & Pytorch& && &&\\ %hline
    & MXNet& && &&\\ %hline
    & CNTK& && &&\\ %hline
    & CoreML& && &&\\ %hline
    & Sklearn& && &&\\ \hline
    
    %LSTM
     \multirow{6}{*}{\rotatebox[origin=c]{90}{\parbox[c]{1cm}{\centering \textbf{LSTM}}}} 
    & Keras& && &&\\ %hline
    & Pytorch& && &&\\ %hline
    & MXNet& && &&\\ %hline
    & CNTK& && &&\\ %hline
    & CoreML& && &&\\ %hline
    & Sklearn& && &&\\ 
    			\bottomrule
    		\end{tabular}  
		%\end{adjustbox}	
	\end{subtable}
	%}
	\end{adjustbox}	
\end{table}

==> tables/tbl_parameters.tex <==
\begin{table*}
\large

\caption{Hyperparameters used for training and converting models. \emph{Input:} Input shape of the model, \emph{Output:} Output shape, \emph{TBatch:} Training batch size, \emph{Tepochs:} Training epochs, \emph{CPbatch:} Conversion and prediction batch size, \emph{Cepochs:} Conversion epochs, \emph{Opt:} Optimization used for training, \emph{Mom:} Momentum, \emph{LR:} Learning Rate, \emph{Dropout:} Dropout Rate.}
\label{validationTable}
\begin{adjustbox}{width=0.75\linewidth,center}
\begin{tabular}{c|c|c|c| c | c | c | c| c| c| c| c} %\toprule
%\rowcolor{gray!15}
\textbf{Model} & \textbf{Input} & \textbf{Output} & \textbf{Tbatch} & \textbf{Tepochs} & \textbf{CPbatch} & \textbf{Cepochs}&\textbf{Mom} &\textbf{Opt}&\textbf{LR}&\textbf{Dropout}\\%\midrule

\hline

%\hline
\rowcolor{gray!10}
\textbf{LeNet-5} &(None, 28, 28, 6)&(None, 10)& 128&50 & 128 & 128&9e-1&sgd&5e-2&-\\

%\hline
\textbf{ResNet-18} & (None, 32, 32, 3)&(None, 10)& 128&50& 128&128 &9e-1&sgd&1e-1&-\\

%\hline
\rowcolor{gray!10}

\textbf{VGG-16}  &(None, 32, 32, 3) &(None, 10)& 128&50 & 128 & 128&9e-1&sgd&1e-1&5e-1\\

\textbf{LSTM}  &(None, 250, 64) &(None, 1)& 250&50 & 128&128&-&Adam&1e-3&5e-1\\
\rowcolor{gray!10}
\textbf{GRU}  &(None, 250, 64) &(None, 1)& 250&50 & 128&128& -&Adam&1e-3&5e-1\\
%\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

%% https://github.com/pytorch/pytorch/issues/42653
% RuntimeError: Unsupported: ONNX export of operator adaptive_avg_pool2d, since output size is not factor of input size. Please feel free to request support or submit a pull request on PyTorch GitHub.
